Discriminating Between Similar Nordic Languages

Automatic language identification is a challenging problem. Discriminating between closely related languages is especially difficult. This paper presents a machine learning approach for automatic language identification for the Nordic languages, which often suffer miscategorisation by existing state-of-the-art tools. Concretely we will focus on discrimination between six Nordic languages: Danish, Swedish, Norwegian (Nynorsk), Norwegian (Bokm{\aa}l), Faroese and Icelandic.

==> original-latex-from-project/data.tex <==

\section{Data acquisition}
The first step when constructing a language classifier is to gather a data set. For this purpose I wrote a small script using the Wikipedia API for Python.\footnote{\url{https://pypi.org/project/wikipedia/}}\\

With the script I was able to download the summaries for randomly chosen Wikipedia articles in each of the languages which are saved to as raw text to 6 {\tt .txt} files of about 10MB each.\\

After the initial cleaning, which i will describe in the next section, the data set contains just over 50K sentences in each of the language categories. I chose to select two data sets with exactly 10K and 50K sentences respectively from the raw data set. In this way the data sets we will work with are balanced, containing the same number of data points in each language category.\\

Throughout this report we split these data sets, reserving 80\% for the training set and 20\% for the test set we use when evaluating the models.

\subsection{Data cleaning}
In this section I will briefly describe how the data set is initially cleaned and how sentences are extracted from the raw data.

\paragraph{Extracting sentences:}

The first thing we want to do is to divide the text into sentences.
This is generally a non-trivial thing to do. My approach is to first split the raw string by line break.
This roughly divides the text into paragraphs with some noise which we filter out in the last step.\\

We then extract shorter sentences with the sentence tokenizer ({\tt sent\_tokenize}) function from the NLTK\cite{nltk} python package. This does a better job than just splitting by {\tt '.'} due to the fact that abbreviations, which can appear in a legitimate sentence, typically include a period symbol.

\paragraph{Cleaning characters}
The initial data set have a lot of characters that do not belong to the alphabets of the languages we work with. Often the Wikipedia pages for people or places contain the name in the original language. For example a summary might contain Chinese or Russian characters which are arguably irrelevant for the purpose of discriminating between the Nordic languages.\\

To make the feature extraction simpler, and to reduce the size of the vocabulary, I chose to make the raw data lowercase and strip all characters with are not part of the standard alphabet of the six languages.\\

In this way we only accept the following character set
\begin{verbatim}
'abcdefghijklmnopqrstuvwxyzáäåæéíðóöøúýþ '
\end{verbatim}
and replace everything else with white space before continuing to extract the features.
For example the raw sentence
\begin{verbatim}
'Hesbjerg er dannet ved sammenlægning
 af de 2 gårde Store Hesbjerg
 og Lille Hesbjerg i 1822.'
\end{verbatim}
will after this initial cleanup be reduced to
\begin{verbatim}
'hesbjerg er dannet ved sammenlægning
 af de gårde store hesbjerg
 og lille hesbjerg i ',
\end{verbatim}
We thus make the assumption that capital letters, numbers and characters outside this character set do not contribute much information relevant for language classification.


==> original-latex-from-project/discussion.tex <==
\section{Conclusion}
In this section I will sum up the results of the paper and provide some suggestions for further work.\\

We have used the dimensionality reduction techniques PCA and t-SNE to make visualizations of feature vectors obtained by making a one-hot encoding with character bi-grams and with the two modes from FastText.\\

These unsupervised techniques was able to separate the sentences from Wikipedia into different clusters.
Without any prior knowledge about the actual language of each sentence these techniques indicated that the six languages can be divided into three main language categories: (1) Danish Nynorsk Bokmål (2) Faroese Icelandic and (3) Swedish.\\

We then compared four different "classical" models: K nearest Neighbors, Logistic regression, Naive Bayes and a linear support vector machines with two neural network architectures: Multilayer perceptron and a convolutional neural network.\\

Generally the supervised models had the largest errors when discriminating between languages belonging to either of the language groups mentioned above.\\

For the "classical" models we saw that Logistic Regression and support vector machines achieved better performance than KNN and Naive Bayes, where the latter performed the worst. This was true in all cases irrespective of the method of feature extraction.\\

Additionally we saw that when we used feature vectors from the FastText skipgram model the classification models achieved better results than when using either FastText cbow or character n-grams.\\

Generally we saw that increasing the number of data points lead to better performance. When comparing the CNN with the "classical" models however the CNN performed better than any of the other models even when trained on less data points. In this way i seems that the CNN is able to learn more from less data when compared to the other models.\\

We saw that when we tested the two best performing models, FastText supervised and CNN, on the dataset from Tatoeba the accuracies dropped quite a lot. We showed that using character n-grams as features instead of words increased the performance for the FastText supervised classifier. By also training FastText on the Tatoeba dataset as well as the Wikipedia dataset resulted in an additional increase in performance.


\subsection{Ideas for improvements}
Here I will provide a couple of ideas for extensions of the work presented in this paper.
\begin{itemize}
  \item \textbf{Hyper parameter optimization:}
  Especially for the neural networks it could be interesting to see if additional tuning of the hyper parameters could result in better performance. One obvious extension would be to try and stacking convolutional layers on top of each other. I briefly looked at this but did not manage to make a rigorous investigation as the training time increased substantially when adding more layers.
  \item \textbf{Implement a two step classification approach.}
  The paper "Discriminating Similar Languages:
  Evaluations and Explorations" \cite{DSLEvaluation} mentions that in the 2014 edition of the DSL competition, the best result achieved an accuracy of 95.7\%. The winning team used a two step approach where their algorithm first classified the language group an then the actual language. The team used a linear support vector machines with words and characters as features.\\
  Inspired by this result I propose to construct a classification algorithm which first discriminates between the major language groups before making a prediction about the actual language with a dedicated classifier. In this way one could treat discriminating between Danish and Bokmål or Faroese and Icelandic as a binary classification problem and see if performance would increase.\\
\end{itemize}




%
% \textbf{Training times}: A major hurdle during the project was the long training times for the different models. Especially the neural networks took several hours to train


==> original-latex-from-project/featureextraction.tex <==
\section{Feature extraction}

In this section I will begin with a brief explanation of how the data is initially cleaned and then go on to explain how the features are extracted.\\

There are several ways of converting text into feature vectors suitable for input for the classification algorithms.
In this paper we compare the performance of encoding the sentences using character level n-grams and compare these results with feature vectors obtained using FastText.

\subsection{Bag of Words and one-hot encoding}
According to \cite{BagOfTricks} a simple and efficient base line for sentence classification is to represent sentences as a of words (BoW) and train a linear classifier.\footnote{The paper proposes logistic regression or an SVM} Here first a brief explanation of the BoW model. \\

Using words as features the first step of doing the BoW representation is to split each sentence into individual words. Continuing the example above the sentence would be split into.

\begin{verbatim}
['hesbjerg','er','dannet','ved',
'sammenlægning','af','de','gårde',
'store','hesbjerg','og','lille',
'hesbjerg','i']
\end{verbatim}

We proceed to make a dictionary over all the words in the the corpus (every word in the complete dataset) counting the frequency by which the each word appears. We can now sort the words by their frequency and in this way we can assign each word to a unique integer.

\begin{verbatim}
[2442,    3, 1513,   39,
 4819,   17,   30, 8684,
  189, 2442,    2,  617,
 2442,    1]
\end{verbatim}

Here we see that {\tt 'i', 'og'} and {\tt 'er' } are the most frequent words in the corpus.

Now for the one-hot encoding we construct a feature vector which has the dimension of the vocabulary and is zero everywhere except in the component corresponding to the integer which we have mapped the word onto as seen above. \\

When using individual word the vocabulary, and thus the dimension of the feature vector for each sentence, increases rapidly with the size of the dataset. In the example above using only 1000 sentences pr language the vocabulary consists of 26695 words and if use 50k sentences in each language the vocabulary grows to  368493!

\subsection{n-grams}

Apart from the large vocabulary, an obvious limitation of the bag of words model described above if that it does not take into account the relative position of each word.\\

A way to remedy this is to use character n-grams as features. An n-gram is constructed by regarding $n$ consecutive tokens (here either words or characters) as the features. An n-gram of size one is called a uni-gram and an n-gram of size 2 is called a bi-gram and so forth.\\

Continuing the example sentence above a bi-gram representation would look like

\begin{verbatim}
['he','es','sb','bj','je','er','rg','g ',
 ' e','er','r ',' d','da','an','nn','ne',
 'et','t ',' v','ve','ed','d ',' s','sa',
 'am','mm','me','en','nl','læ','æg','gn',
 'ni','in','ng','g ',' a',...]
\end{verbatim}

An advantage of using a character level representation instead of a word level is a drastic reduction in the vocabulary size. Since we only accept 40 characters a one-hot encoding using character level uni-grams would have at most 40 components while bi-grams would have a vocabulary of $40^2 = 1600$  and for trigrams the vocabulary would grow to  $40^3 = 64000$.\\

In this project we will compare the performance of a bag of words encoding using character level uni-grams and bi-grams with feature vectors obtained from using FastText.

\subsection{Using FastText}

The methods described above are quite simple and in this project i will also compare the above method with FastText which is a library for creating word embeddings developed by Facebook \cite{BagOfTricks}. \\

In the paper "Enriching Word Vectors with Subword Information" \cite{EnrichingWordVectors} the authors explain how FastText extracts feature vectors from raw text data. FastText makes word embedding using one of two model architectures: continuous bag of words (cbow) or the continuous skipgram model.\\

The skipgram and cbow models are first proposed in \cite{EfficientWordRepresentations} which is the paper introducing the word2vec model for word embeddings. FastText builds upon this work by proposing an extension to the skipgram model which takes into account subword information.\\

Both models use a neural network to learn word embedding from using a context windows consisting of the words surrounding the current target word. The CBOW architecture predicts the current word based on the context, and the skipgram predicts surrounding words given the current word.\cite{EfficientWordRepresentations} We see an illustration of this in Figure \ref{cbowskipgram}.

\begin{figure}[h!]
  \centering
  \includegraphics[width = 225pt]{figs/cbowskipgram}
  \caption{Diagram of the cbow and skipgram models.}
  \label{cbowskipgram}
\end{figure}



% % The order of context words does not influence prediction (bag-of-words assumption)
% Works by minimizing the-likelihood
%
% \begin{align}
% \sum_{t=1}^{T}\sum_{c}^{c \in C_t} \log p(w_c|w_t)
% \end{align}


% Skipgram vs continued bag of words.

% However, term frequencies are not necessarily the best representation for the text. Common words like "the", "a", "to" are almost always the terms with highest frequency in the text. Thus, having a high raw count does not necessarily mean that the corresponding word is more important. To address this problem, one of the most popular ways to "normalize" the term frequencies is to weight a term by the inverse of document frequency, or tf–idf. Additionally, for the specific purpose of classification, supervised alternatives have been developed to account for the class label of a document.[4] Lastly, binary (presence/absence or 1/0) weighting is used in place of frequencies for some problems (e.g., this option is implemented in the WEKA machine learning software system).


==> original-latex-from-project/introduction.tex <==
\section{Introduction}
Automatic language identification is a challenging problem and especially discriminating between closely related languages is one of the main bottlenecks of state-of-the-art language identification systems.\cite{DSL2014}\\

The problem has been investigated in recent work \cite{DSLEvaluation}\cite{DSL2015} which discuss the results from two editions of the "Discriminating between Similar Languages (DSL) shared task". Over the two editions of the DSL shared task different teams competed to develop the best machine learning algorithms to discriminate between the languages in a corpus consisting of 20K sentences in each of the languages: Bosnian, Croatian, Serbian, Indonesian, Malaysian, Czech, Slovak, Brazil Portuguese, European Portuguese, Argentine Spanish, Peninsular Spanish, Bulgarian and Macedonian.\\

In this project we will develop a machine learning based pipeline for automatic language identification for the Nordic languages. Concretely we will focus on discrimination between the six Nordic languages: Danish, Swedish, Norwegian (Nynorsk), Norwegian (Bokmål), Faroese and  Icelandic.\\

We will explore different ways of extracting features from a corpus of raw text data consisting of summaries from Wikipedia in the respective languages and continue to evaluate the performance of a selection of machine learning models.\\

Concretely we will compare the performance of classic machine learning models such as Logistic Regression, Naive Bayes, Support vector machine, and K nearest Neighbors with more contemporary neural network approaches such as Multilayer Perceptrons (MLP)  Convolutional Neural Networks (CNNs).\\

After evaluating these models on the Wikipedia dataset we will continue to evaluate the best models on a Dataset from a different domain in order to investigate how well the models generalize when classifying sentences from a different domain.


%  and a Long Short Term Memory architecture (LSTM).\\
% Feed Forward Neural networks or


==> original-latex-from-project/models.tex <==
\section{Models}
Now the feature vectors are extracted we can begin to develop classification models. In this section I will briefly go through the theory of for classic machine learning models and continue to explain the core concepts of the neural network architectures

The problem of assigning one of mutually exclusive languages to a sentence is an example of a multi class classification problem. Since we have gathered a dataset with which we can train our models we are dealing with supervised learning.

Let us start with developing a bit of notation.
We are provided with a set of data points $\mathcal{X}$ together with an associated set of labels $\mathcal{Y}$.
We can define our \emph{dataset} $\mathcal{D}$ the as follows
\begin{align}
\mathcal{D} = \{(\mathbf{x}_i,y_i)|\mathbf{x}_i\in\mathcal{X},y_i\in\mathcal{Y}\}
\end{align}

where we have that the data points and labels are defined by
\begin{align}
\mathcal{X}&=\{\mathbf{x}_1, \mathbf{x}_2, \mathbf{x}_3, \cdots,\mathbf{x}_n\} \qquad \mathbf{x}_i \in \mathbf{R}^{m}  \\
\mathcal{Y}&=\{y_1, y_2, y_3, \cdots,y_n\} \qquad y_i \in C
\end{align}
Where $C$ is the set of possible language categories, in this case the set
\begin{align}
  C = \{"dk", "sv", "nn", "nb", "fo", "is"\}
\end{align}
Now our aim is to construct a function $f$ of some parameters $\theta$ such that given a datapoint $\mathbf{x}$ the function returns the predicted label $\hat{y}$

\begin{align}
 \hat{y} = f_\theta (\mathbf{x})
\end{align}

Now the predicted label might not be correct and we need a measure of how wrong our model is over the whole dataset. One common error function is the mean squared error (MSE) cost function.

\begin{align}
  E_{\text{MSE}} = \frac{1}{n}\sum_i^n (\hat{y}_i - y_i)^2
\end{align}
Later for the training of the neural networks with keras we will use the categorical cross entropy (CCE) which is given by.
\begin{align}
  E_{\text{CCE}} = -\frac{1}{n}\sum_i^n \sum_{c\in C} y_{i,c}\ln \hat{y_{i,c}}
\end{align}

\subsection{Baseline models}

As mentioned in \cite{BagOfTricks}, simple baseline models for text classification are for example logistic regression and support vector machines. In this project I will also test how the performance of the K Nearest Neighbors algorithm and a Naive Bayes classifier.
%
% In addition to the neural networks I would like to test how more conventional Machine Learning models compare to models based on neural networks.

\subsubsection{K Nearest Neighbors}
Perhaps the simplest model to understand is the K Nearest Neighbors classification algorithm. Here we calculate the distance from a test example which we want to label to its $k$ "Nearest Neighbors". The distance $d$ between the test example $\mathbf{x}$ and a labeled data point $\mathbf{x}_{\text{train}}$ in the training set is the conventional euclidean distance.

\begin{align}
d=\sqrt{\sum_{i=1}^m (x_i-x_{\text{train}_i})^2}
\end{align}

The algorithm calculates the distance $c$ between a test point $\mathbf{x}$ to all other data points in the training set. Then we simply assign the most common label to $\mathbf{x}$ among its $k$ nearest neighbors. In this project and for the results to be presented later we have set $k=3$.

\subsubsection{Linear support vector machines}
Support vector machine is all about finding the maximal margin hyperplanes.

Any hyper plane in the feature space can be written as points satisfying
\begin{align}
    \mathbf{w}\cdot\mathbf{x} + \mathbf{b} = 0
\end{align}

We want to find the two parallel hyperplanes where the distance between them is at large as possible.
The functional form of the linear support vector machine then becomes
\begin{align}
    \hat{y} = \text{sign}(\mathbf{w}\cdot \mathbf{x} + b)
\end{align}
Where we define
\begin{align}
    \mathbf{w} = \sum_i \alpha y_i \mathbf{x}_i
\end{align}
Where $\alpha_i$ is only non-zero for the support  vectors $\mathbf{x}_i$. Thus the aim thus the aim is to minimize $||\mathbf{w}||$ since the width between the two supporting hyperplanes is proportional to $1/||\mathbf{w}||$

\subsubsection{Logistic Regression}
Contrary to the k nearest neighbors and support vector machine algorithm described above in Logistic regression we calculate the probability that $\mathbf{x}$ belongs to the language $C_k$ as
\begin{align}
p(C_k|\mathbf{x}) = f(\mathbf{x}) = \frac{1}{1+e^{\theta^T \mathbf{x}}}
\end{align}
The predicted label of the logistic regression model is then given by
\begin{align}
  \hat{y} = \text{argmax}_k p(C_k|\mathbf{x})
\end{align}
The method for finding the parameters $\theta$ which minimizes the error is gradient decent which is given by
\begin{align}
  \theta_{t+1} = \theta_t + \eta \nabla E
\end{align}

\subsubsection{Naive Bayes}
% Our goal is to find the probability of belonging to a language class $C_k$. given a sentence $\mathbf{x}$ $p(C_k|\mathbf{x})$.  The famous Bayes' theorem states that
%
% \begin{align}
% p(A|B) = \frac{p(B|A)p(A)}{p(B)}
% \end{align}

Our goal is to find the probability of belonging to a language class $C_k$. We can use Bayes' theorem here to find the probability $p(C_k|\mathbf{x})$ of a language class $C_k$ given a feature vector $\mathbf{x}$. Using Bayes Theorem we get

\begin{align}
p(C_k|\mathbf{x}) = \frac{p(C_k)}{p(\mathbf{x})} p(\mathbf{x}|C_k)
\label{bayes1}
\end{align}

Now the prior $p(\mathbf{x})$ is a constant and so it $p(C_k)$ if the number of data points in each of the language categories are equal, as is the case here. We can rewrite $p(\mathbf{x}|C_k)$ using the assumption that the features $x_i$\footnote{This is the "naive" part of Naive Bayes} are independent we can write.
\begin{align}
p(\mathbf{x}|C_k) = p(C_k) \prod_i p(x_i|C_k)
\label{bayes2}
\end{align}
By using eq. $\ref{bayes2}$ in eq. $\ref{bayes1}$ and selecting the largest probability we get the prediction by.

\begin{align}
\hat{y} = \underset{k}{\text{argmax  }} p(C_k) \prod_i p(x_i|C_k)
\end{align}
% \begin{align}
% p(C_k|\mathbf{x}) \propto p(C_k) \prod_i p(x_i|C_k)
% \end{align}

\subsection{Neural Networks}
In this section I will go through the basic theory behind the two neural network architectures Multi layer Perceptrons and convolutional neural networks.


\subsubsection{Feed Forward Neural Networks}
Arguably the simplest neural network if the Multi Layer Perception MLP. A MLP consists of at least 3 layers where the first is the input layer which have the same number of nodes as the feature vector we feed into the network. The last layer is the output layer which always have the same number of nodes at the number of different classes, six in this cave.

In the MLP we use dense layers as the hidden layers, this means that all the nodes in a layer are connected to all nodes in the next layer.

In each layer we take the output from the previous layer and multiply each component with a set of weights, the values of which we optimize during training, sum them up and pass the result to a nonlinear activation function.

The activation function in the hidden layers is the rectified linear unit or ReLU function
\begin{align}
  \text{ReLU}(z)= \text{max}(0,z)
\end{align}

The activation function final layer is the softmax function
\begin{align}
  \text{softmax}(z)_i= \frac{e^z_i}{\sum_{j=1}^k e^z_j}
\end{align}
where $k$ is the number of different classes.

\subsubsection{Convolutional Neural Networks}

While every layer in the MLP is densely connected such that each of the nodes in a layer is connected to all nodes in the next layer, in a convolution neural network we use one or more convolutional layers.

Convolutional Neural networks are very popular for image recognition but they can also be used for text classification \cite{textcnn_google}.

\begin{figure}[h!]
  \centering
  \includegraphics[width = 200pt]{figs/cnn_diagram}
  \caption{Diagram of Convolutional Neural network.}
  \label{cnn}
\end{figure}

The basic premise of a convolutional layer is illustrated in figure \ref{cnn}\footnote{Source: \url{https://realpython.com/python-keras-text-classification/}}. In a CNN you have a filter which slides over the input. The CNN then takes the dot product of the weights of the filter and the corresponding input features, before applying the activation function. The kernel size is a hyper parameter which can be optimized by experimentation which we will also do later.



==> original-latex-from-project/results.tex <==
\section{Results}
In this section I will present the results from running the various classification models on the Wikipedia dataset and then proceed to investigate how well these models perform on a dataset from a different domain.

\subsection{Baseline With langid.py}

As a baseline to compare the performance of the models in this word I would like to compare with an out of the box language classification system. "langid.py: An Off-the-shelf Language Identification Tool." \cite{langID} is such a tool.\\

Out of the box langid.py comes with with a pretrained model which covers 97 languages. The data for langid.py comes from from 5 different domains: government documents, software documentation, newswire, online encyclopedia and an internet crawl.\\

I have written a program to test how well langid.py performed on the Wikipedia dataset using the the python API.\footnote{\url{https://pypi.org/project/langid/}}\\

Since langid.py returned the language id "no" (Norwegian) on some of the data points i chose to restrict langid.py to only be able to return either "nn" (Nynorsk) or "nb" (Bokmål) as predictions. It is a quite peculiar feature of the Norwegian language that there exist two different written languages but three different language codes.

\begin{figure}[h!]
  \centering
  \includegraphics[width = 200pt]{figs/langid}
  \caption{Confusion matrix with results from langid.py on the full dataset with 300K data points. }
  \label{langid_confusion_matrix}
\end{figure}

In Figure \ref{langid_confusion_matrix} we see the confusion matrix for the langid.py classifier. The largest errors are between Danish and Bokmål and between Faroese and Icelandic. We see that langid.py was actually able to correctly classify most of the Danish data points however approximately a quarter of the data points in Bokmål was incorrectly classified as Danish and just under and eighth was classified as Nynorsk.\\

Furthermore langid.py correctly classified most of the Icelandic data points however over half of the data points in Faroese was incorrectly classified as Icelandic.

\subsection{Baseline with linear models.}

In the Figure \ref{baseline-results-10k} we see the results for running the models on a dataset with 10K data points in each language category. We see that the models in general perform better if we use character level bi-grams instead of uni-grams (individual) characters.\\

Also we see that logistic regression and support vector machines outperform Naive Bayes and K nearest neighbors in all cases. Furthermore for all models we get the best performance if we use the skipgram model from FastText.\\

If we compare the cbow mode from FastText with character level bi-grams we see that the cbow model is on par with bi-grams for the KNN and Naive Bayes classifiers while bi-grams outperform the cbow for Logistic Regression and support vector machines.\\

\begin{figure}[h!]
  \centering
  \begin{tabular}{ l | c | r }
    \hline
    Model               & Encoding  & Accuracy \\
    \hline
    Knn                 & cbow &  0.780\\
    Log-Reg             & cbow &  0.819\\
    Naive Bayes         & cbow &  0.660\\
    SVM                 & cbow &  0.843\\
    Knn                 & skipgram &  0.918\\
    Log-Reg             & skipgram &  \textbf{0.929}\\
    Naive Bayes         & skipgram &  0.840\\
    SVM                 & skipgram &  \textbf{0.928}\\
    Knn                 & char bi-gram  & 0.745\\
    Log-Reg             & char bi-gram  & 0.907\\
    Naive Bayes         & char bi-gram  & 0.653\\
    SVM                 & char bi-gram  & 0.905\\
    Knn                 & char uni-gram  & 0.620\\
    Log-Reg             & char uni-gram  & 0.755\\
    Naive Bayes         & char uni-gram  & 0.614\\
    SVM                 & char uni-gram  & 0.707\\
    \hline
  \end{tabular}
  \caption{Overview of results for the dataset with 10K data points in each language.}
  \label{baseline-results-10k}
\end{figure}

\subsection{Results with neural networks.}
In the following we evaluate the initial results for the neural network architectures which can be seen in Figure \ref{keras-results}. Here we compare the result of doing character level uni- and bi-grams using the Multilayer Perceptron and Convolutional Neural Network. We see that the CNN performs the best, achieving an accuracy of 95.6\% when using character bi-grams. Both models perform better using bi-grams than individual characters as features while the relative increase in performance is greater for the MLP model.

\begin{figure}[h!]
  \centering
  \begin{tabular}{ l | c | r }
    \hline
    Model               & Encoding  & Accuracy \\
    \hline
    MLP                 & char bi-gram &  0.898 \\
    CNN                 & char bi-gram & \textbf{0.956} \\
    % LSTM                & char bi-gram & 60k & 0.933 \\
    MLP                 & char uni-gram &  0.697\\
    CNN                 & char uni-gram  & 0.942 \\
    % LSTM                & char uni-gram & 60k &  \\
    \hline
  \end{tabular}
  \caption{Overview of results for the neural network models for the dataset with 10K data points in each language.}
  \label{keras-results}
\end{figure}


\subsection{Increasing the size of the dataset.}
Usually the performance of supervised classification models increase with more training data. In this section I have increased amount of training data to 50K sentences in each of the language categories. Due to much longer training times I choose to only rerun the "baseline models" with the skipgram encoding from FastTest which we saw achieved the highest accuracy.

\begin{figure}[h!]
  \centering
  \begin{tabular}{ l  c | r }
    \hline
    Model               & Encoding & Accuracy \\
    \hline
    Knn                 & skipgram & 0.931\\
    Logistic Regression & skipgram  & \textbf{0.933}\\
    Naive Bayes         & skipgram  & 0.806\\
    SVM                 & skipgram& 0.925\\
    \hline
  \end{tabular}
  \caption{Overview of results for the dataset with 50K data points in each language.}
  \label{results-sklearn300k}
\end{figure}

As can be seen in Figure \ref{results-sklearn300k} the accuracies for the logistic regression model and the K nearest neighbors algorithm improved by including more data, however not by much. Unexpectedly the accuracies for the support vector machine and naive Bayes actually dropped a bit by including more data.\\

Even when including five times the amount of data the best result, logistic regression with an accuracy of 93.3\%, is still worse than for the Convolutional Neural Network trained on 10K data points in each language.\\

In Figure \ref{results-keras-300k} we see the results for running the neural networks on the larger dataset. Both models improve by increasing the amount of data and the Convolutional Neural Network reached an accuracy of 97\% which is the best so far.

\begin{figure}[h!]
  \centering
  \begin{tabular}{ l c | r }
    \hline
    Model               & Encoding & Accuracy \\
    \hline
    MLP                 & char bi-gram  & 0.918\\
    CNN                 & char bi-gram  & \textbf{0.970}\\
    \hline
  \end{tabular}
  \caption{Overview of results for the dataset with 50K data points in each language.}
  \label{results-keras-300k}
\end{figure}

% In Figure \ref{training} we see a plot of the accuracy during training on the training and validation set respectively. We see that the accuracy on the validation set follows the accuracy on the training set more closely for the CNN than for the MLP.

% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}[b]{100pt}
%         \includegraphics[width=\textwidth]{figs/training_MLP}
%         \caption{Training accuracy MLP}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{100pt}
%         \includegraphics[width=\textwidth]{figs/training_CNN}
%         \caption{Training accuracy CNN}
%     \end{subfigure}
%     \caption{Accuracy on test and validation set during training of the different neural networks on the full dataset with 50K data points in each language.}
%     \label{training}
% \end{figure}

In Figure \ref{confusion_matrix-big-cnn} we see the confusion matrix for the convolutional Neural Network trained on the full Wikipedia dataset with 300K data points pr language. We see that the largest classification errors still happens between Danish, Bokmål and Nynork as well as between Icelandic and Faroese. \\

\begin{figure}[h!]
  \centering
  \includegraphics[width = 200pt]{figs/confusion_CNN}
  \caption{Confusion matrix with results from the convolutional neural network on the full datasetwith 50K data points in each language.}
  \label{confusion_matrix-big-cnn}
\end{figure}

\subsection{Optimizing the kernel size.}
In attempt to optimize the CNN i tried to look at different kernel sizes (between 1 and 11) for character level uni- bi- and trigrams. I tested on the dataset with 10K sentences in each language since the training time for a single CNN was several hours and it would have taken several days to train on the full dataset even using cloud resources in Google Colab. We see the results in Figure \ref{kernel_sizes}.\\

\begin{figure}[h!]
  \centering
  \includegraphics[width = 225pt]{figs/KernelSizes}
  \caption{Accuracy for different kernel sizes for the Constitutional Neural Network.}
  \label{kernel_sizes}
\end{figure}

\subsection{Using FastText supervised}

FastText can also be used for be trained supervised and be used for Classification. In the Paper Bag of Tricks for Efficient Text Classification \cite{BagOfTricks} the authors show that FastText can obtain performance on par with methods inspired by deep learning, while being much faster on a selection of different tasks in Tag prediction and Sentiment Analysis. The confusion matrix from running the FastText supervised classifier can be seen in Figure \ref{fasttext_supervised}. We see that FastText is on par with the CNN\\


\begin{figure}[h!]
  \centering
  \includegraphics[width = 225pt]{figs/fasttext_supervised}
  \caption{Confusion matrix with results from a supervised FastText model on the full dataset with 300K datapoints.}
  \label{fasttext_supervised}
\end{figure}

\subsection{Reflections.}
At this point I it beneficial to take a step back and look at what we have done so far. We have developed a selection of different models and our results to far indicate that the FastText supervised model and the CNN both give quite good results on the Wikipedia dataset with accuracies over 97\%. \\

In the rest of this section I would like to investigate the cases there these classifiers fail and try if I can find common patters. Also i will test the models on a dataset which they have not been trained on to investigate how well the models generalize to data from a different domain than Wikipedia. \\


\subsection{Looking at failure cases}
Now having achieved quite good results with FastText and the CNN I now look a bit more closely at the sentences which were misclassified by both models. \\

As a first observation the misclassified sentences tend to be shorter than the correctly classified ones. In Figure \ref{faliurelengthdist} I have plotted the distribution of the length, defined as the number of characters after the data cleaning procedure as defined in a previous section. The mean length of the sentences in the test set is 104.74 characters with a standard deviation of 65.39 while it is only 48.91 characters with a deviation  of 37.27. \\

\begin{figure}[h!]
    \centering
    \includegraphics[width=200pt]{figs/faliurelengthdist}
    \caption{Distribution of sentence lengths.}
    \label{faliurelengthdist}
\end{figure}

Generally the misclassified sentences fall into the categories: Very short sentences, names, mathematical content and sentences with many foreign words.\\

\textbf{Mathematical equations}:
A substantial (and useful) part of Wikipedia is related to mathematics and equations are common on these pages. My Wikipedia scraper did not filter out mathematical equations which appear in the dataset as in the examples below. \\

\begin{verbatim}
displaystyle n lambda eff cdot t
displaystyle a frac a cot frac pi simeq a
displaystyle a b c a cdot b a cdot c ab ac
\end{verbatim}

\textbf{Foreign Words}:
Another common type of misclassified sentences with a lot of foreign words. In the dataset this commonly happened with English words. Below are some examples of misclassified sentences where most or all word are from foreign languages. \\

\begin{verbatim}
art garfunkel all i know skywriter
 watermark

mémoires de la société des antiquaires
du nord fjögur bindi

avatar the last airbender prins zuko

the fifth dimension up up and away
\end{verbatim}
% heimsnet e mbwa mobile broadband wireless access
% y is yhat dk
%  y is yhat nb
% y dk yhat fo
%  y nb yhat fo


\textbf{Names}: Another common failure case is sentences that contain only names of people or locations. Examples are
\begin{verbatim}
  romain rolland
  henry morton stanley
  anna karin
\end{verbatim}
% y is yhat fo
% y sv yhat fo
% y is yhat fo

It is not surprising that these cases are hard to classify since names are usually spelled the same way irrespective of language. \\

\textbf{Danish and Bokmål}:
One of the largest error categories was sentences on Danish or Bokmål misclassified as the other language.\\

This is not surprising sine these two languages are very closely related and often the difference between them is an alternative spelling of a single word in a sentence. \\

The examples below are in Bokmål but was classified as Danish. The first sentence is in indistinguishable from danish except from the alternative spelling of the single word  "magesekken" which would be "mavesækken" in Danish. \\

The Second sentence would be hard or impossible for a native speaker to distinguish since the there is no difference between this sentence in the two languages.Finally for the third example the difference is only two characters in the word "sommerfuglhager" which in danish would be spelled as "sommerfuglehaver".

\begin{verbatim}
(1) hos mennesket har magesekken et
    volumet ca

(2) klubben har hjemmebane på slettebakken
    hvor de også har et klubbhus

(3) en dyrepark kan derfor også omfatte
    for eksempel akvarier terrarier
    sommerfuglhager og fuglehus
\end{verbatim}

\subsection{Evaluating the models on another dataset}
It would be interesting to see how the two best performing models generalize by testing on a dataset different from the they have been trained on (the Wikipedia dataset).\\

I downloaded an additional dataset from Tatoeba\footnote{{\tt tatoeba.org/}} which is a large database of user provided sentences and translations. In Figure \ref{tatoebasentprlang} we see the number of sentences in each language for all sentences in the Tatoeba dataset. Observe that we have very few samples in Nynorsk and Faroese.\\

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width =\textwidth]{figs/tatoebasentprlang}
      \caption{Distribution of the number of sentences in each language in the tatoeba dataset.}
      \label{tatoebasentprlang}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width =\textwidth]{figs/taboeba-faliurelengthdist}
      \caption{Distribution of the length of  sentences tatoeba dataset.}
      \label{tatoebalengths}
    \end{subfigure}
        \caption{Distribution of the lengths and language classes of Tatoeba sentences.}
\end{figure}

The language used in the Tatoeba dataset is different from the language used in Wikipedia. The Tatoeba dataset mainly consists of sentences written in everyday language. Below we see some examples from the Danish part of the Tatoeba dataset.
\begin{verbatim}
Hvordan har du det?

På trods af al sin rigdom
og berømmelse, er han ulykkelig.

Vi fløj over Atlanterhavet.

Jeg kan ikke lide æg.

Folk som ikke synes at latin er det
smukkeste sprog, har intet forstået.
\end{verbatim}

The confusion matrix for the FastText supervised model and the CNN, which are both trained on the full Wikipedia dataset and then evaluated on the Tatoeba dataset can be seen in Figure \ref{tatoeba-confuss}. Both models use the same setting that produced good results on the Wikipedia dataset.

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/tatoeba-langid}
        \caption{Langid.py}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/tatoeba-fasttext}
        \caption{fasttext classifier }
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/tatoeba-cnn}
        \caption{Convolutional neural network}
    \end{subfigure}
    \caption{Confusion matrices for the tatoeba dataset }
    \label{tatoeba-confuss}
\end{figure}

We see that the performance drops quite a lot when shifting to another domain. For reference the accuracy of langid.py on this dataset is 80.9\% so FastText actually performs worse than the baseline with an accuracy of 75.5\% while the CNN is a bit better than the baseline with an accuracy of 83.8 \% \\

One explanation for the drop in performance is that the sentences in the Tatoeba dataset is significantly shorter than the sentences in the Wikipedia dataset as seen in Figure \ref{tatoebalengths}. As we saw in the previous section both models tend to misclassify shorter sentences more often than longer sentences. This and the fact that the "genre" of sentences are different might explain why the models trained on the Wikipedia dataset does not generalize too well to the Tatoeba dataset without a drop on performance.\\

The CNN uses character bi-grams as features while, with the standard settings, FastText uses only individual words to train. The better performance of the CNN might indicate that character level n-grams are more useful features for language identification than words alone.\\

To test this I changed the setting of FastText to train using only character level n-grams in the range 1-5 instead of individual words. In Figure \ref{fasttextcharngram} we see the confusion matrix for this version of the FastText model. This version still achieved 97.8\% on the Wikipedia test set while improving the accuracy on the Tatoeba dataset from 75.4\% to 85.8\% which is a substantial increase.\\

Thus using character level features seem to improve the FastText models ability to generalize to sentences belonging to a domain different from the one it has been trained on.

\begin{figure}[h!]
    \centering
    \includegraphics[width=200pt]{figs/fasttextcharngram}
    \caption{Confusion matrix for FastText trained using only characterlevel n-grams on the Wikipedia dataset and evaluated on the tatoeba dataset.}
    \label{fasttextcharngram}
\end{figure}


\subsection{Retraining on the combined dataset}
To improve the accuracy on the Tatoeba dataset I decided to retrain the FastText model on a combined dataset consisting of datapoints from
both the Wikipedia and Tatoeba dataset.\\

The FastText model achieved an accuracy of 97.2\% on this combined dataset and an accuracy of 93.2\% when evaluating this model on the Tatoeba test set alone - the confusion matrix can be seen in Figure \ref{retrain-confuss}.\\

As was the case with the Wikipedia dataset the misclassified sentences tend to be shorter than the average sentence in the dataset. In Figure \ref{retrain-lengths} we see the distribution of sentence lengths for the Tatoeba test set along with the misclassified sentences.\\

 In the Tatoeba test set the mean length of sentences is 37.66 characters with a standard deviation of 17.91 while the mean length is only 29.70 characters for the misclassified sentences with a standard deviation of 9.65. This again supports the conclusion that shorter sentences are harder to classify.

\begin{figure}[h!]
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width=200pt]{figs/retrain}
      \caption{Confusion matrix for FastText trained using only characterlevel n-grams on the combined Wikipedia/Tatoeba dataset and evaluated on the tatoeba dataset.}
      \label{retrain-confuss}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/faliurelengthdist_tatoeba}
        \caption{Distribution of sentence lengths Tatoeba testset along with the misclassified sentences.}
     \label{retrain-lengths}
    \end{subfigure}
\end{figure}


% Not surprisingly we see a substantial increase in performance when including datapoints

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=200pt]{figs/retrain}
%     \caption{Confussion matrix for fastText trained using only characterlevel ngrams on the combined Wikipedia/Tatoeba dataset and evaluated on the tatoeba dataset.}
%     \label{retrain}
% \end{figure}



% \begin{figure}
%   \centering
%   \includegraphics[width = 300pt]{figs/encoding_dimension}
%   \caption{The the performance of the different models.}
%   \label{encodings}
% \end{figure}
%
%
% \begin{figure}
%   \centering
%   \includegraphics[width = 300pt]{figs/skipgram}
%   \caption{The the performance of the different models.}
%   \label{skipgram}
% \end{figure}


==> original-latex-from-project/visualization.tex <==
\section{Visualization}
In this section we will try to develop some intuition about the dataset by making different visualizations.

\subsection{Character distributions}
One obvious thing to look at is how frequent each character appears in each language.
In Figure \ref{chardist}\footnote{Some of the characters miss Diacritics i could not find a solution for matplotlib to handle there characters.} I have plotted the frequency by which each character appears for each language in the corpus, in Figure \ref{chardistnorm} i have normalized the distribution by dividing each occurrence of a character with the total number of times that character appear in the dataset.\\
\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/chardist}
        \caption{Character frequencies}
        \label{chardist}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figs/chardistnorm}
        \caption{Normalized character frequencies}
        \label{chardistnorm}
    \end{subfigure}
    \caption{Frequency of each character in each language. The character are ordered along the x-axis according to the frequency by which they appear in the dataset. }
    %\label{chardist}
\end{figure}

Interestingly the most frequent character {\tt e} is much less frequent in Faroese and Icelandic than in the other languages. Not surprisingly the character  {\tt ð} only appears in Faroese and Icelandic while it is much more frequent in Icelandic. The character {\tt þ} is exclusive to Icelandic and  {\tt ö} almost only appears in Swedish. We could potentially use the information about the relative frequencies of characters in the models.


\subsection{Principal Component analysis and t-SNE}
To gain additional insight on how the different word embedding capture important information about each of the language classes I thought it would be interesting to try and visualize the embeddings using two different techniques for dimensionality reduction.\\

No matter which way we choose to extract the feature vectors they belong to a high dimensional feature space and in order to do visualization we need to project the feature vectors down to 2d space.\\

To do this I have implemented two different methods: Principal Component Analysis (PCA) which i will compare with T-distributed Stochastic Neighbor Embedding (t-SNE).
Here we will begin with a brief explanation of the two techniques and proceed with an analysis of the results.

\paragraph{Pricipal Component Analysis}

The first step is to calculate the covariance matrix of the dataset.
The components of the covariance matrix is given by

\begin{align}
K_{X_i,X_j} = E[(X_i - \mu_i )(X_j -  \mu_j)]
\end{align}

where $X_{i}$ is the $i$th component of the feature vector and $\mu_{i}$ is the mean of that component.

In matrix form we can thus write the covariance matrix as
\begin{align}
K(\mathbf{x},\mathbf{z}) =
\begin{bmatrix}
    \text{cov}(x_1,z_1) &  \dots  & \text{cov}(x_1,z_n) \\
    \vdots & \ddots     & \vdots \\
    \text{cov}(x_n,z_1) & \dots  & \text{cov}(x_n,z_n) \\
\end{bmatrix}
\end{align}
The next step is to calculate the eigenvectors and eigenvalues of the covariance matrix by solving the eigenvalue equation.
\begin{align}
\det (K v-\lambda v) = 0
\end{align}
The eigenvalues are the variances along the direction of the eigenvectors or "Principal Components". To project our dataset onto 2D space we select the two eigenvectors largest associated eigenvalue and project our dataset onto this subspace.\\

In Figure \ref{pca} we see the result of running the PCA algorithm on the wikipedia dataset where we have used character level bigrams as features as well as the cbow and skipgram models from FastTest.\\


\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/pcachar2}
        \caption{Character bigram}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/pcacbow1}
        \caption{Fasttext cbow}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/pcaskipgram1}
        \caption{Fasttext skipgram}
    \end{subfigure}
    \caption{Dimensionality reduction using PCA}
    \label{pca}
\end{figure}

In the figure for encoding with character level bi-grams the PCA algorithm resulted in two elongated clusters. Without giving any prior information about the language of each sentences the PCA is apparently able to discriminate between Danish, Swedish, Nynorsk and Bokmål on one side and Faroese and Icelandic on the other since the majority of the sentences in each language belong to either of these two clusters. With the FastText implementations we observe three clusters.\\

For both cbow and skipgram we see a distinct cluster of Sweedish sentences. When comparing the two FastText models we see that the t-SNE algorithm with skipgrams seems to be able to separate the Faroese and Icelandic data points to a high d ecree compared with the cbow model. Also for the cluster identified with the sentences with Danish, Bokmål and Nynorsk the skipgram models seem seem to give a better separation, however to a lesser degree than with the two former languages.

\paragraph{t-SNE}

The T-distributed Stochastic Neighbor Embedding method was first proposed in 2008 in the paper "Visualizing Data using t-SNE"\cite{tsne}.

In the paper the authors explain the theory behind the algorithm which I  will make a brief summary of here.

Suppose you pick a data point $x_i$, then the probability of picking another data point $x_j$ as a neighbor to $x_i$ is given by
\begin{align}
p_{ji}= \frac{\exp (|| x_i - x_j ||^2/2\sigma_i^2 )}{\sum_{k\neq i} \exp (|| x_i - x_k ||^2/2\sigma_i^2 )}
\end{align}

Now having this probability distribution the goal is to find the low-dimensional mapping of the data points $x_i$ which we denote $y_i$ follow a similar distribution. To solve what is referred to as the "crowding problem" the t-SNE algorithm uses the "Student t-distribution" which is given by
\begin{align}
q_{ij}= \frac{ (1+|| y_i - y_j ||^2 )^{-1}}{\sum_{k\neq l} (1+|| y_k - y_l ||^2 )^{-1}}
\end{align}
Now finally for optimizing this distribution is done by using gradient decent on the "Kullback-Leibler divergence" which is given by
\begin{align}
\frac{\delta C}{\delta y_i}= 4 \sum_j (p_{ij} - q_{ij})(y_i-y_j)(1+ || y_i - y_j ||^2  )^{-1}
\end{align}

The result from running the t-SNE algorithm on the wikipedia dataset can be seen in Figure \ref{tsne}. As was the case with the PCA algorithm it appears that the encoding with FastText seem to capture the most relevant information to discriminate between the languages, especially the skipgram mode seems to do a good job in capturing relevant information.\\

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/tsnechar2}
        \caption{Character bigram}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/tsnecbow1}
        \caption{Fasttext cbow}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figs/tsneskipgram1}
        \caption{Fasttext skipgram}
    \end{subfigure}
    \caption{Dimensionality reduction using t-SNE}
    \label{tsne}
\end{figure}


Here we recover some interesting information about the similarity of the languages. The data points in Bokmål lies in between those in Danish and Nynorsk while Icelandic and Faroese have their own two clusters which are separated from the three former languages. \\

This is in good agreement with what we already know about the languages. Interestingly the Swedish data points and quite scattered and the t-SNE is not able to make a coherent Swedish cluster.\\

This does not however mean that the Swedish datapoint are not close in the original space. Some care is needed when interpreting the plot since t-SNE groups together data points such that neighboring points in the input space will tend to be neighbors in the low dimensional space.\\

If points are separated in input space, t-SNE would like to separate them in the low dimensional space however it does not care how far they are separated. So clusters that are far away in the low dimensional space are not necessarily far away in the input space.

% Unlike PCA, axes in the low dimensional space don't have a particular meaning. In fact, one could arbitrarily rotate the low dimensional points and the t-SNE cost function wouldn't change. Furthermore, t-SNE doesn't construct explicit mappings relating the high dimensional and low dimensional spaces.
%
% Rather, the relevant information is in the relative distances between low dimensional points. t-SNE captures structure in the sense that neighboring points in the input space will tend to be neighbors in the low dimensional space.
%
% But, some care is needed because larger distances can't necessarily be interpreted. If points are separated in input space, t-SNE would like to separate them in the low dimensional space. But, it doesn't care how far they are (unlike PCA, MDS, or isomap, for example). Another issue is that t-SNE sometimes breaks continuous segments of data into pieces and artificially separates them, particularly at low perplexity settings. See here for a good example. t-SNE is framed as a visualization tool rather than a pre-processing or analysis tool, and doing things like clustering in the low dimensional space can be dangerous because of these issues. The upshot is that distorting distances sometimes lets t-SNE produce good 2/3d visualizations of data that are intrinsically higher dimensional.
%
% One way that t-SNE visualizations can be useful is by combining them with external information. This can reveal patterns in the data that we may not have been aware of. For example, the t-SNE papers show visualizations of the MNIST dataset (images of handwritten digits). Images are clustered according to the digit they represent--which we already knew, of course. But, looking within a cluster, similar images tend to be grouped together (for example, images of the digit '1' that are slanted to the left vs. right). And, points that appear in the 'wrong' cluster are sometimes actually mislabelled in the original dataset, or ambiguously written (e.g. something between '4'and a '9').

